Conspiracy Brokers: Understanding the Monetization of YouTube Conspiracy Theories

Conspiracy theories are increasingly a subject of research interest as society grapples with their rapid growth in areas such as politics or public health. Previous work has established YouTube as one of the most popular sites for people to host and discuss different theories. In this paper, we present an analysis of monetization methods of conspiracy theorist YouTube creators and the types of advertisers potentially targeting this content. We collect 184,218 ad impressions from 6,347 unique advertisers found on conspiracy-focused channels and mainstream YouTube content. We classify the ads into business categories and compare their prevalence between conspiracy and mainstream content. We also identify common offsite monetization methods. In comparison with mainstream content, conspiracy videos had similar levels of ads from well-known brands, but an almost eleven times higher prevalence of likely predatory or deceptive ads. Additionally, we found that conspiracy channels were more than twice as likely as mainstream channels to use offsite monetization methods, and 53% of the demonetized channels we observed were linking to third-party sites for alternative monetization opportunities. Our results indicate that conspiracy theorists on YouTube had many potential avenues to generate revenue, and that predatory ads were more frequently served for conspiracy videos.

==> aggregator_analysis.tex <==
%\vznote{I'm putting what I found about aggregates and affiliates here, feel free to edit. If it doesnt belong here feel free to move it wherever. Once I have all the numbers all the wording will be better, I'm still trying to figure out how to organize this part} 
%\subsubsection{Aggregator Sites} 
%\label{sec:gameaggs}
%Game aggregator sites were one of the most frequent individual types of advertisers we observed. Highly overrepresented in the control set \tlnote{Since they're mostly in the control set, they're less relevant for this study since they don't contribute much to funding conspiracy videos. I'd mostly remove this section; if useful we can keep a sentence saying that predatory advertising also exists outside of conspiracy content and mention aggregators as an example (but that's hardly surprising or novel)} \vlnote{Agree}, these sites all hosted numerous links to apps and flash games, or hosted the games themselves. The sites commonly use bright colors and exciting thumbnails often seen in other advertisements for children. These sites seem to monetize through direct referrals to app developers or by running advertisements in games. While these sites do not target conspiracy videos specifically, we included them in the discussion because their deceptive practices and potential impact on children warrant further investigation. 

%In the United States, advertisers are restricted from using behavioral tracking for children under 13 without explicit parental consent \cite{kidtracking}. However, even the most well-established aggregators do not provide clear protections to prevent this tracking. \textit{mafa.com} states that they do not perform tracking on areas of the site where a user has identified their age as under 13, but most of the site has no age-gating whatsoever. \textit{Poki} claim different tracking practices for their main site and PokiKids, but offer no controls or even suggestions to keep children off of the main site. Two others, \textit{ufreegames} and \textit{Vigoo}, imply that they may be targeting parents and thus indirectly targeting children as well. The last, \textit{lagged.com} simply claims the site is only for users aged 13 and older, but does not include any protections or notifications of this on their site. 



%\vznote{I'll mainly be discussing the games aggregators, I'll need to procure the full list of all things classified as aggregator if possible, if not I can change this to just be games aggregators}
%We found that in the top 90\% of ad views, 38 domains pointed to by ads were aggregator sites focused on Gaming. 25 of these actually allow you to play games on the site, while the other 13 simply host links to the app store or game 'reviews' that are essentially just advertisements for a game. Most of the playable games are clones of popular mobile games. They are often monetized by serving advertisements before the game runs. 1 domain \textit{games-4-free.com} is monetized using affiliate links.
%We can tell what companies own 5 of the games platforms: Mafa, Poki, Vigoo, ufreegames, and Lagged. Mafa is a longstanding game site that hosts flash games. Poki's privacy policy also state that they serve behavioral advertisements on their general site, on the site for children under 13 \textit{PokiKids} they only serve contextual advertisements and cap the number of ads seen \vznote{reference(https://poki.com/en/c/privacy-statement) }
%\textit{ufreegames.com} and \textit{vigoo.com} imply that they may be targeting parents of children and indirectly children. \textit{ufreegames.com} states on their about page that:"Our ultimate aim is to provide fun time online for moms and their kids with varieties of different games of multiple levels." \vznote{reference(https://www.ufreegames.com/about.html)}
%\textit{lagged.com} however states that their site and games are only for users aged 13 or over \vznote{reference https://lagged.com/privacy}

%\cbnote{I think the stuff below is interesting, but unsure how to succinctly discuss and fit into the paper} \vznote{Maybe move the specific sites out into the appendix or citations and just mention that there were certain games that had either no guarantee of their content being malware free and another group of games that connect to and gets data from a site that hosts and communicates with MobiGame. I think we can take out the infinite scrolling stuff and keep the platforms with "lability" because that fits in with youtube allowing advertisements that lead to risky sites}
%We found three separate site layouts that were replicated on multiple domains. More research is needed to find out if these ads are a result of coordinated monetization attempts:

%MobiGame: Of note 13 of the platforms' links seemingly redirect to the google app store. All their urls link to the directory /ext/, mostly /ext/gmgt/. These all look to be all put out from the same company and seem to have at one time installed either a program or browser extension. When we viewed the source of the site using curl, we found that each of the game's urls pointed to mbdl219.com. According to alien vault, this url hosts 1 malicious file, and communicates to 13 files, all of which are Win32:Mobigame, which is Adware that disguises itself as an Android emulator. \vznote{reference https://otx.alienvault.com/indicator/domain/mbdl219.com}\cite{doyle_2016} It is noted that on the bottom of the websites of these platforms, they have a link that tells you how to uninstall the MobiGame extension and program. Interestingly one domain \textit{myarcadegames.app} that does not share the layout also has an uninstall page that implies it installs a browser extension, though at the time of viewing we could not find any evidence that they currently install any browser extensions.

%Infinite Scrolling: 3 of the games platforms: \textit{kolagames.com}, \\ \textit{hoopgame.net} and \textit{9bob.net} feature an assortment of games that you can infinitely scroll through. When inspecting their source, they often use assets from other games platforms with infinite scrolling pages, \vznote{good way of saying leading us to believe} that these all belong to the same group.

%"Lability" Clause [sic]: 2 of the games platforms \textit{kacle.com} and \textit{freegames.nz} explicitly state that "they do not warrant that the content is free of viruses or harmful components." in the mispelled liability section of their privacy policies \vznote{reference(https://www.kacle.com/privacy.html and https://freegames.nz/privacy.html)}. Upon viewing the source code on their game's page, we found that the games were embedded iframes that originates from the Infinite Scrolling platforms. We believe they may be owned by the same people who own the Infinite Scrolling platforms.

==> case_study.tex <==

These advertisements additionally obscure ownership through multiple tiers of shell companies and different hosting pages. As a case study, the advertiser \textit{get-ryoko.com} sells a product also hosted on \textit{getryoko.com} and \textit{ryokorouter.com}. The product has a 1.7/5 rating on Google reviews, with frequent complaints of failure to deliver on promises, but displays 4.5/5 stars on their main pages. \textit{Ryoko} is managed by a parent company, \textit{Muama}, that also advertised a translation device with a 2.1/5 rating, \textit{translatorenence.com}. \textit{Muama} in turn is owned by the broader internet retail company, \textit{ekomlita.com}, which claims to be a generic internet retail platform. 

A clear understanding of these practices would require much deeper investigation, but our preliminary analysis suggests an ecosystem where companies are able to market poor quality products by obscuring ownership through a combination of shell companies and deceptive affiliate advertising. \textit{Ryoko} can claim any undelivered promises were made by the affiliate marketer, and the affiliate can claim they were just advertising a third-party product. \textit{Muama} can mitigate harm caused by \textit{Ryoko's} poor reputation by selling other products like \textit{Enence} through a separate company, and \textit{Ekomlita} can claim they are a retail platform without direct involvement in any individual product. Ultimately, this increases customer confusion and shields \textit{Ryoko}, \textit{Muama}, and \textit{Ekomlita} from moderation by Google. Each affiliate appears to be a separate advertiser unrelated to the product's official company, enabling \textit{Ryoko} to successfully carry out deceptive campaigns while mitigating the impact of any enforcement actions against individual affiliates or parent companies.

==> figures/category_std_resids.tex <==
\begin{tabular}{lrr}
\toprule
Dataset & Conspiracy & Control \\
Category                &            &         \\
\midrule
Aggregator sites        &      -59.0 &    59.0 \\
Information Media       &       2.90 &   -2.90 \\
Merchant                &      -23.4 &    23.4 \\
Self-improvement        &        106 &    -106 \\
Special Interest Groups &       3.23 &   -3.23 \\
\bottomrule
\end{tabular}

==> figures/category_table.tex <==
\begin{tabular}{llrr}
\toprule
               Category &    Dataset & Ad Count & Percent of Dataset \\
\midrule
       Aggregator sites & conspiracy &      288 &           1.03\textbackslash ,\textbackslash \% \\
       Aggregator sites &    control &  10.9\textbackslash ,k &           13.6\textbackslash ,\textbackslash \% \\
      Information Media & conspiracy &      165 &           0.59\textbackslash ,\textbackslash \% \\
      Information Media &    control &      367 &           0.46\textbackslash ,\textbackslash \% \\
               Merchant & conspiracy &  20.9\textbackslash ,k &           74.5\textbackslash ,\textbackslash \% \\
               Merchant &    control &  66.2\textbackslash ,k &           82.1\textbackslash ,\textbackslash \% \\
       Self-improvement & conspiracy &  5.69\textbackslash ,k &           20.3\textbackslash ,\textbackslash \% \\
       Self-improvement &    control &  1.63\textbackslash ,k &           2.02\textbackslash ,\textbackslash \% \\
Special Interest Groups & conspiracy &      561 &           2.00\textbackslash ,\textbackslash \% \\
Special Interest Groups &    control &  1.39\textbackslash ,k &           1.73\textbackslash ,\textbackslash \% \\
\bottomrule
\end{tabular}

==> figures/subcat_table.tex <==
\begin{tabular}{llrr}
\toprule
        Sub-category &    Dataset & Ad Count & Percent of Dataset \\
\midrule
  Alternative Health & conspiracy &  2.03\textbackslash ,k &           7.25\textbackslash ,\textbackslash \% \\
  Alternative Health &    control &      556 &           0.69\textbackslash ,\textbackslash \% \\
              Beauty & conspiracy &      749 &           2.67\textbackslash ,\textbackslash \% \\
              Beauty &    control &  1.31\textbackslash ,k &           1.63\textbackslash ,\textbackslash \% \\
  Business/Marketing & conspiracy &  3.12\textbackslash ,k &           11.1\textbackslash ,\textbackslash \% \\
  Business/Marketing &    control &  1.92\textbackslash ,k &           2.38\textbackslash ,\textbackslash \% \\
           Education & conspiracy &      687 &           2.45\textbackslash ,\textbackslash \% \\
           Education &    control &      912 &           1.13\textbackslash ,\textbackslash \% \\
          Education  & conspiracy &      517 &           1.84\textbackslash ,\textbackslash \% \\
          Education  &    control &      306 &           0.38\textbackslash ,\textbackslash \% \\
         Electronics & conspiracy &  1.39\textbackslash ,k &           4.95\textbackslash ,\textbackslash \% \\
         Electronics &    control &  1.38\textbackslash ,k &           1.71\textbackslash ,\textbackslash \% \\
       Entertainment & conspiracy &  1.53\textbackslash ,k &           5.46\textbackslash ,\textbackslash \% \\
       Entertainment &    control &  2.27\textbackslash ,k &           2.82\textbackslash ,\textbackslash \% \\
             Fashion & conspiracy &      887 &           3.16\textbackslash ,\textbackslash \% \\
             Fashion &    control &  5.54\textbackslash ,k &           6.87\textbackslash ,\textbackslash \% \\
           Financial & conspiracy &      893 &           3.18\textbackslash ,\textbackslash \% \\
           Financial &    control &  3.45\textbackslash ,k &           4.28\textbackslash ,\textbackslash \% \\
          Food/Drink & conspiracy &  1.79\textbackslash ,k &           6.40\textbackslash ,\textbackslash \% \\
          Food/Drink &    control &  2.67\textbackslash ,k &           3.31\textbackslash ,\textbackslash \% \\
               Games & conspiracy &  3.45\textbackslash ,k &           12.3\textbackslash ,\textbackslash \% \\
               Games &    control &  11.0\textbackslash ,k &           13.7\textbackslash ,\textbackslash \% \\
Gold/precious metals & conspiracy &      316 &           1.13\textbackslash ,\textbackslash \% \\
Gold/precious metals &    control &      509 &           0.63\textbackslash ,\textbackslash \% \\
          Government & conspiracy &     16.0 &           0.06\textbackslash ,\textbackslash \% \\
          Government &    control &      164 &           0.20\textbackslash ,\textbackslash \% \\
          Home goods & conspiracy &      683 &           2.44\textbackslash ,\textbackslash \% \\
          Home goods &    control &  3.57\textbackslash ,k &           4.43\textbackslash ,\textbackslash \% \\
          Industrial & conspiracy &      314 &           1.12\textbackslash ,\textbackslash \% \\
          Industrial &    control &      570 &           0.71\textbackslash ,\textbackslash \% \\
           Insurance & conspiracy &      892 &           3.18\textbackslash ,\textbackslash \% \\
           Insurance &    control &      805 &           1.00\textbackslash ,\textbackslash \% \\
           Lifestyle & conspiracy &  1.56\textbackslash ,k &           5.56\textbackslash ,\textbackslash \% \\
           Lifestyle &    control &      807 &           1.00\textbackslash ,\textbackslash \% \\
      Major Retailer & conspiracy &  1.20\textbackslash ,k &           4.29\textbackslash ,\textbackslash \% \\
      Major Retailer &    control &  6.91\textbackslash ,k &           8.58\textbackslash ,\textbackslash \% \\
             Medical & conspiracy &  1.96\textbackslash ,k &           6.98\textbackslash ,\textbackslash \% \\
             Medical &    control &  12.0\textbackslash ,k &           14.9\textbackslash ,\textbackslash \% \\
           Political & conspiracy &      124 &           0.44\textbackslash ,\textbackslash \% \\
           Political &    control &      649 &           0.81\textbackslash ,\textbackslash \% \\
            Software & conspiracy &  2.70\textbackslash ,k &           9.62\textbackslash ,\textbackslash \% \\
            Software &    control &  21.1\textbackslash ,k &           26.2\textbackslash ,\textbackslash \% \\
           Streaming & conspiracy &      121 &           0.43\textbackslash ,\textbackslash \% \\
           Streaming &    control &      359 &           0.45\textbackslash ,\textbackslash \% \\
      Transportation & conspiracy &      197 &           0.70\textbackslash ,\textbackslash \% \\
      Transportation &    control &      721 &           0.89\textbackslash ,\textbackslash \% \\
\bottomrule
\end{tabular}

==> figures/subcategory_std_resid.tex <==
\begin{tabular}{lrr}
\toprule
Dataset & Conspiracy & Control \\
Subcategory               &            &         \\
\midrule
Alternative Health   &       62.8 &   -62.8 \\
Beauty               &       11.4 &   -11.4 \\
Business/Marketing   &       60.9 &   -60.9 \\
Education            &       16.2 &   -16.2 \\
Education            &       24.7 &   -24.7 \\
Electronics          &       30.3 &   -30.3 \\
Entertainment        &       21.4 &   -21.4 \\
Fashion              &      -22.1 &    22.1 \\
Financial            &      -7.54 &    7.54 \\
Food/Drink           &       23.1 &   -23.1 \\
Games                &      -4.71 &    4.71 \\
Gold/precious metals &       8.52 &   -8.52 \\
Government           &      -5.10 &    5.10 \\
Home goods           &      -14.3 &    14.3 \\
Industrial           &       6.91 &   -6.91 \\
Insurance            &       25.9 &   -25.9 \\
Lifestyle            &       45.7 &   -45.7 \\
Major Retailer       &      -22.9 &    22.9 \\
Medical              &      -33.2 &    33.2 \\
Political            &      -6.02 &    6.02 \\
Software             &      -56.8 &    56.8 \\
Streaming            &      -0.12 &    0.12 \\
Transportation       &      -2.78 &    2.78 \\
\bottomrule
\end{tabular}

==> figures/top_ads_by_dataset.tex <==

\begin{tabular}{llr}
\toprule
   Dataset &                     Advertiser & Times Seen \\
\midrule
conspiracy &          https://hero-wars.com &    3.20\textbackslash ,k \\
conspiracy &  https://go.publishinglife.com &        867 \\
conspiracy &    https://pharmacy.amazon.com &        714 \\
conspiracy &         https://www.amazon.com &        678 \\
conspiracy &           https://www.usaa.com &        518 \\
conspiracy &        https://www.youtube.com &        348 \\
conspiracy &       https://healthyto120.com &        305 \\
conspiracy &      https://superzoomtech.com &        259 \\
conspiracy &   https://www.totaladblock.com &        257 \\
conspiracy & https://www.bookofremedies.org &        254 \\
   control &    https://pharmacy.amazon.com &    10.5\textbackslash ,k \\
   control &   https://www.totaladblock.com &    8.43\textbackslash ,k \\
   control &         https://www.amazon.com &    5.93\textbackslash ,k \\
   control &           https://us.romwe.com &    2.84\textbackslash ,k \\
   control &             https://adgone.org &    2.63\textbackslash ,k \\
   control &         https://ourfunzone.com &    1.93\textbackslash ,k \\
   control &        https://zonedgamers.com &    1.83\textbackslash ,k \\
   control & https://capitaloneshopping.com &    1.37\textbackslash ,k \\
   control &     https://www.ufreegames.com &    1.25\textbackslash ,k \\
   control &          https://liveouter.com &    1.22\textbackslash ,k \\
\bottomrule
\end{tabular}


==> figures/top_ads_by_sub_cat.tex <==
% Will add if needed

